Efficient Digital Quadratic Unconstrained Binary Optimization Solvers for SAT Problems

Boolean satisfiability (SAT) is a propositional logic problem of determining whether an assignment of variables satisfies a Boolean formula. Many combinatorial optimization problems can be formulated in Boolean SAT logic -- either as k-SAT decision problems or Max k-SAT optimization problems, with conflict-driven (CDCL) solvers being the most prominent. Despite their ability to handle large instances, CDCL-based solvers have fundamental scalability limitations. In light of this, we propose recently-developed quadratic unconstrained binary optimization (QUBO) solvers as an alternative platform for 3-SAT problems. To utilize them, we implement a 2-step [3-SAT]-[Max 2-SAT]-[QUBO] conversion procedure and present a rigorous proof to explicitly calculate the number of both satisfied and violated clauses of the original 3-SAT instance from the transformed Max 2-SAT formulation. We then demonstrate, through numerical simulations on several benchmark instances, that digital QUBO solvers can achieve state-of-the-art accuracy on 78-variable 3-SAT benchmark problems. Our work facilitates the broader use of quantum annealers on noisy intermediate-scale quantum (NISQ) devices, as well as their quantum-inspired digital counterparts, for solving 3-SAT problems.

==> util/maths.def.tex <==
%\newcommand{\Bmath}[1]{\mbox{\boldmath${#1}$\unboldmath}}
\newcommand{\Bmath}[1]{\mbox{\bf {#1}}}
\newcommand{\bd}[1]{\mbox{\boldmath $#1$}}
% \newcommand{\Bmath}[1]{\mbox{\boldmath {#1}}}
\newcommand{\Bc}{\Bmath{c}}
\newcommand{\Bb}{\Bmath{b}}
\newcommand{\Bd}{\Bmath{d}}
\newcommand{\BD}{\Bmath{D}}
\newcommand{\Be}{\Bmath{e}}
\newcommand{\Bi}{\Bmath{i}}
\newcommand{\Bj}{\Bmath{j}}
\newcommand{\BI}{\Bmath{I}}
\newcommand{\BL}{\Bmath{L}}
\newcommand{\BG}{\Bmath{G}}
\newcommand{\BB}{\Bmath{B}}
\newcommand{\Bg}{\Bmath{g}}
\newcommand{\Bh}{\Bmath{h}}
\newcommand{\Bt}{\Bmath{t}}
\newcommand{\BR}{\Bmath{R}}
\newcommand{\BT}{\Bmath{T}}
\newcommand{\Bx}{\Bmath{x}}
\newcommand{\Bs}{\Bmath{s}}
\newcommand{\Br}{\Bmath{r}}
\newcommand{\By}{\Bmath{y}}
\newcommand{\Bw}{\Bmath{w}}
\newcommand{\BBw}{\overline{\Bmath{w}}}
\newcommand{\BTw}{\widetilde{\Bmath{w}}}
\newcommand{\BSw}{\Bmath{w}_*}
\newcommand{\BW}{\Bmath{W}}
\newcommand{\BBW}{\overline{\Bmath{W}}}
\newcommand{\BSW}{\Bmath{W}_*}
\newcommand{\BV}{\Bmath{V}}
\newcommand{\BU}{\Bmath{U}}
\newcommand{\Bu}{\Bmath{u}}
\newcommand{\Bv}{\Bmath{v}}
\newcommand{\Bq}{\Bmath{q}}
\newcommand{\BF}{\Bmath{F}}
\newcommand{\BP}{\Bmath{P}}
\newcommand{\BK}{\Bmath{K}}
\newcommand{\BM}{\Bmath{M}}
\newcommand{\BN}{\Bmath{N}}
\newcommand{\Bf}{\Bmath{f}}

\newcommand{\Bone}{\Bmath{1}}
\newcommand{\Bzero}{\Bmath{0}}

\newcommand{\CZ}{{\cal Z}}


\newcommand{\g}{\gamma_1}
\newcommand{\gt}{\gamma_2}

\newcommand{\Te}{T_e(\g; N,\ell)}
\newcommand{\TE}{T_{N,N_1}(\g)}
\newcommand{\Ten}{T_e(\g; N,N-1)}
\newcommand{\Tenf}{T'_e(\g; N,N-1)}
\newcommand{\Tenff}{T''_e(\g; N,N-1)}
\newcommand{\Tenfn}{T'_e(\g^0; N,N-1)}
\newcommand{\Tenffn}{T''_e(\g^0; N,N-1)}
\newcommand{\Tenn}{T_e(\g^0; N,N-1)}
\newcommand{\Ts}{T_s(\g)}
\newcommand{\Tsq}{T_{s,1}(\g)}
\newcommand{\Tsl}{T_{s,2}(\g)}
\newcommand{\Tu}{T_u(\g; N,\ell)}
\newcommand{\ld}{\ln(\cdot)}

\newcommand{\Ss}{S_{N-1}}
\newcommand{\Sso}{S^0_{N-1}}


\newcommand{\Tw}{\tilde{w}}

\newcommand {\de  } {\delta     }      \newcommand {\De  } {\Delta     }
\newcommand {\fr  } {\frac           } \newcommand {\ov  } {\over         }
% \newcommand {\be  } {\beta     } 

\newcommand {\CA  } {{\cal   A }}       
\newcommand {\CB  } {{\cal   B }}       
\newcommand {\CE  } {{\cal   E }}       
\newcommand {\CF  } {{\cal   F }}       
\newcommand {\CH  } {{\cal   H }}       
\newcommand {\CI  } {{\cal   I }}       
\newcommand {\CJ  } {{\cal   J }}       
\newcommand {\CK  } {{\cal   K }}       
\newcommand {\CL  } {{\cal   L }}       
\newcommand {\CD  } {{\cal   D }}       
\newcommand {\CN  } {{\cal   N }}
\newcommand {\CO  } {{\cal   O }}
\newcommand {\CQ  } {{\cal   Q }}
\newcommand {\CP  } {{\cal   P }}      
\newcommand {\CS  } {{\cal   S }}       
\newcommand {\CT  } {{\cal   T }}       
\newcommand {\CX  } {{\cal   X }}       
\newcommand {\CR  } {{\cal   R }}       
\newcommand {\CY  } {{\cal   Y }}       
\newcommand {\CG  } {{\cal   G }}       
\newcommand {\CV  } {{\cal   V }}  
\newcommand {\CW  } {{\cal   W }}       

\newcommand {\CU  } {{\cal   U }}       



\newcommand {\kk  } {\kappa     } 
\newcommand {\ka  } {\kappa     } 
\newcommand {\ev  } {\equiv                          }

\newcommand {\lh  } {\left(                          }
\newcommand {\rh  } {\right)                         }

\newcommand {\e    } {\!+\!                  }
\newcommand {\m    } {\!-\!                  }
\newcommand {\hsc } {\hspace*{1cm}   }

\newcommand{\BGamma}{{\bf \Gamma}}
\newcommand{\BPi}{{\bf \Pi}}
\newcommand{\BPsi}{{\bf \Psi}}
\newcommand{\BPhi}{{\bf \Phi}}


% Define argmax. argmin
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}


\newcommand{\A}{{\cal A}}
\newcommand{\GG}{{\cal G}}

\newcommand{\RR}{{\mathbb{R}}}
\newcommand{\NN}{{\mathbb{N}}}
\newcommand{\EE}{{\mathbb{E}}}


\newcommand{\BAR}[1]{{\bf{#1}}}

\def\x{{\Bmath x}}
\def\e{{\Bmath e}}
\def\c{{\Bmath c}}
\def\p{{\Bmath p}}
\def\w{{\Bmath w}}
\def\m{{\Bmath m}}
\def\a{{\Bmath a}}
\def\b{{\Bmath b}}
\def\g{{\Bmath g}}
\def\y{{\Bmath y}}
\def\z{{\Bmath z}}
\def\f{{\Bmath f}}
\def\s{{\Bmath s}}
\def\d{{\Bmath d}}
\def\n{{\Bmath n}}
\def\h{{\Bmath h}}
\def\z{{\Bmath z}}
\def\t{{\Bmath t}}
\def\r{{\Bmath r}}
\def\w{{\Bmath w}}
\def\u{{\Bmath u}}
\def\q{{\Bmath q}}
\def\v{{\Bmath v}}

\def\D{{\Bmath D}}
\def\M{{\Bmath M}}
\def\P{{\Bmath P}}
\def\R{{\Bmath R}}
\def\I{{\Bmath I}}
\def\H{{\Bmath H}}
\def\l{{\Bmath L}}
\def\B{{\Bmath B}}
\def\E{{\Bmath E}}
\def\Z{{\Bmath Z}}
\def\A{{\Bmath A}}
\def\X{{\Bmath X}}
\def\G{{\Bmath G}}
\def\C{{\Bmath C}}
\def\Y{{\Bmath Y}}
\def\T{{\Bmath T}}
\def\W{{\Bmath W}}
\def\Q{{\Bmath Q}}
\def\K{{\Bmath K}}
\def\V{{\Bmath V}}


\def\cT{{\cal T}}	
\def\cN{{\cal N}}
\def\cL{{\cal L}}
\def\cW{{\cal W}}
\def\cY{{\cal Y}}
\def\cZ{{\cal Z}}

\newcommand*\diff{\mathop{}\!\mathrm{d}}

\newcommand{\Er}{{\cal E}_{TRN}}
\newcommand{\Eg}{{\cal E}_{GEN}}


%\newcommand{\expectation}[1]{{\mathbb E}\left[ #1 \right]}



==> util/theorem.def.tex <==
\newtheorem{theorem}{Theorem}[section]

\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}   
\newtheorem{conjecture}[theorem]{Conjecture} 
\newtheorem{lemma}[theorem]{Lemma}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{question}[theorem]{Question}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}

% \numberwithin{equation}{section}

% Package for commenting 
\usepackage{xcolor}
\newcommand{\commenttext}[1]{\textcolor{blue}{\text{ #1 }}}
\newcommand{\comment}[1]{\textcolor{blue}{ #1 }}

